DeHiDe: Deep Learning-based Hybrid Model to Detect Fake News using Blockchain

The surge in the spread of misleading information, lies, propaganda, and false facts, frequently known as fake news, raised questions concerning social media's influence in today's fast-moving democratic society. The widespread and rapid dissemination of fake news cost us in many ways. For example, individual or societal costs by hampering elections integrity, significant economic losses by impacting stock markets, or increases the risk to national security. It is challenging to overcome the spreading of fake news problems in traditional centralized systems. However, Blockchain-- a distributed decentralized technology that ensures data provenance, authenticity, and traceability by providing a transparent, immutable, and verifiable transaction records can help in detecting and contending fake news. This paper proposes a novel hybrid model DeHiDe: Deep Learning-based Hybrid Model to Detect Fake News using Blockchain. The DeHiDe is a blockchain-based framework for legitimate news sharing by filtering out the fake news. It combines the benefit of blockchain with an intelligent deep learning model to reinforce robustness and accuracy in combating fake news's hurdle. It also compares the proposed method to existing state-of-the-art methods. The DeHiDe is expected to outperform state-of-the-art approaches in terms of services, features, and performance.

==> ap.tex <==
\appendix
\section{Appendix} 


==> discussion.tex <==
%\section{Discussion}
%\label{sec:disc}





In this section, proposed model is compared with existing methods. \tabref{comp} provides insights into the features provided in the state-of-the-art approaches and the proposed DeHiDe. 
\begin{table}[!htb]
\caption{DeHiDe comparison with state-of-the-art blockchain-based solutions.%\psanote{Paul et al.~\cite{paul2019fake} is missing.}
}
\label{tab:comp}
\resizebox{1\columnwidth}{!}{%
        \begin{tabular}{l|c|c|c|c|c|c|c|c}
        \hline
            \textbf{Features}            &
            
            \begin{tabular}[c]{@{}c@{}}{Chen}\\{et al.~\cite{chen2018towards}} \end{tabular}  &
            
            \begin{tabular}[c]{@{}c@{}}{{Islam}}\\{{et al.~\cite{islam2020newstradcoin}}} \end{tabular} &
            
            \begin{tabular}[c]{@{}c@{}}{Qayyum}\\{et al.~\cite{qayyum2019using}}\end{tabular} &
            
            \begin{tabular}[c]{@{}c@{}}{Shang}\\{et al.~\cite{shang2018tracing}} \end{tabular}  &
            
            \begin{tabular}[c]{@{}c@{}}{Arquam}\\{et al.~\cite{arquam2018blockchain}} \end{tabular}  &
            
            \begin{tabular}[c]{@{}c@{}}{Balouchestani}\\{et al.~\cite{balouchestani2019sanub}}\end{tabular} &
            
            \begin{tabular}[c]{@{}c@{}}{Paul}\\{et al.~\cite{paul2019fake}}\end{tabular} &
            
            \textbf{DeHiDe} \\ \hline\hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{News} \textbf{Broadcasting}\end{tabular} & 
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Ownership} \textbf{Proof}\end{tabular} &
            &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Fake News} \textbf{Detection}\end{tabular} &
            &
            &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Reporters} \textbf{Validation}\end{tabular} & 
            &
            &
            &
            &
            $\bcheck$ &
            $\bcheck$ &
            &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{News} \textbf{Evaluation}\end{tabular} &
            &
            &
            &
            &
            &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Analyst} \textbf{Existence}\end{tabular} & 
            &
            &
            &
            &
            &
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Native User}  \textbf{Importance}\end{tabular} &
            &
            &
            &
            &
            &
            &
            $\bcheck$ &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Random Analyst} \textbf{Selection}\end{tabular} &
            &
            &
            &
            &
            &
            &
            $\bcheck$ &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{DL (NLP)} \textbf{Model}\end{tabular} &
            &
            &
            &
            &
            &
            &
            &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Real-time} \textbf{System}\end{tabular} &
            &
            &
            &
            &
            &
            &
            &
            $\bcheck$ \\ \hline
            
            
            \end{tabular}%
}
\end{table}

From the \tabref{comp}, it can be observed that many features that support better accuracy in detecting fake news and maintaining quality provided in the proposed methodology. In the earlier works, either of blockchain or deep learning models to detect fake news. Here we propose a novel idea combine blockchain with intelligent deep learning models in single architecture for better accuracy. We also propose the criteria to pick the raters in the system without bias. The proposed architecture is currently partially implemented. As future work, we plan to implement a fully functioning network to compare the proposed model's accuracy with architecture proposed in the past.



\iffalse
\begin{table}[!htb]
\caption{DeHiDe comparison with the state-of-the-art approaches.}
%\vspace{-.2cm}
\label{tab:comp}
\resizebox{1\columnwidth}{!}{%
        \begin{tabular}{l|c|c|c|c|c|c|c}
        \hline
            \textbf{Features}            &
            
            \begin{tabular}[c]{@{}c@{}}{{Islam}}\\{{et al.~\cite{islam2020newstradcoin}}} \end{tabular} &
            
            \begin{tabular}[c]{@{}c@{}}{Shang}\\{et al.~\cite{shang2018tracing}} \end{tabular}  &
            
            \begin{tabular}[c]{@{}c@{}}{Arquam}\\{et al.~\cite{arquam2018blockchain}} \end{tabular}  &
            
            \begin{tabular}[c]{@{}c@{}}{Chen}\\{et al.~\cite{chen2018towards}} \end{tabular}  &
            
            \begin{tabular}[c]{@{}c@{}}{Qayyum}\\{et al.~\cite{qayyum2019using}}\end{tabular} &
            
            \begin{tabular}[c]{@{}c@{}}{Balouchestani}\\{et al.~\cite{balouchestani2019sanub}}\end{tabular} &
            
            \textbf{DeHiDe} \\ \hline\hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{News} \textbf{Broadcasting}\end{tabular} & 
            $\bcheck$ & 
            $\bcheck$ &
            $\bcheck$ &
            $\bcheck$ & 
            $\bcheck$ &
            $\bcheck$ & 
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Ownership} \textbf{Proof}\end{tabular} & 
            $\bcheck$ & 
            $\bcheck$ & 
            $\bcheck$ & 
            &
            $\bcheck$ & 
            $\bcheck$ & 
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Detect} \textbf{Fake News}\end{tabular} &
            & 
            $\bcheck$ & 
            $\bcheck$ &     
            & 
            $\bcheck$ & 
            $\bcheck$ & 
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Reporters} \textbf{Validation}\end{tabular} & 
            &
            &
            $\bcheck$ &
            &
            & 
            $\bcheck$ & 
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{News} \textbf{Evaluation}\end{tabular} &
            &
            &
            &
            &
            &
            $\bcheck$ &
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Analyst} \textbf{Existence}\end{tabular} & 
            & 
            & 
            & 
            & 
            & 
            $\bcheck$ & 
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{DL(NLP)} \textbf{Model}\end{tabular} & 
            & 
            & 
            & 
            & 
            &
            & 
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Native User}  \textbf{Importance}\end{tabular} & 
            & 
            & 
            & 
            & 
            &
            & 
            $\bcheck$ \\ \hline
            
            \begin{tabular}[c]{@{}c@{}}\textbf{Analyst Selection} \textbf{Randomness}\end{tabular} & 
            & 
            & 
            & 
            & 
            &
            & 
            $\bcheck$ \\ \hline
        \end{tabular}%
    }
\end{table}
\fi
